Contextual Bandits with Stochastic Experts

We consider the problem of contextual bandits with stochastic experts, which is a variation of the traditional stochastic contextual bandit with experts problem. In our problem setting, we assume access to a class of stochastic experts, where each expert is a conditional distribution over the arms given a context. We propose upper-confidence bound (UCB) algorithms for this problem, which employ two different importance sampling based estimators for the mean reward for each expert. Both these estimators leverage information leakage among the experts, thus using samples collected under all the experts to estimate the mean reward of any given expert. This leads to instance dependent regret bounds of $\mathcal{O}\left(\lambda(\pmb{\mu})\mathcal{M}\log T/\Delta \right)$, where $\lambda(\pmb{\mu})$ is a term that depends on the mean rewards of the experts, $\Delta$ is the smallest gap between the mean reward of the optimal expert and the rest, and $\mathcal{M}$ quantifies the information leakage among the experts. We show that under some assumptions $\lambda(\pmb{\mu})$ is typically $\mathcal{O}(\log N)$, where $N$ is the number of experts. We implement our algorithm with stochastic experts generated from cost-sensitive classification oracles and show superior empirical performance on real-world datasets, when compared to other state of the art contextual bandit algorithms.

==> defs.tex <==
\section{Problem Setting and Definitions}
\label{sec:defs}
We consider a general contextual bandit setting where the task is to compete against a large class of stochastic experts. In the stochastic setting the general contextual bandit problem with $K$ arms is defined as a sequential process for $T$ discrete time-steps~\cite{langford2008epoch}, where $T$ is the time-horizon of interest. At each time $t \in \{ 1,2,\cdots,T\}$ nature draws a vector $(x_t, r_1(t),...,r_K(t))$ from an unknown but fixed probability distribution. Here, $r_{i}(t) \in [0,1]$ is the reward of arm $i$. The context vector $x_t \in \mathcal{X}$ is revealed to the policy-designer, whose task is then to choose an arm out the $K$ possibilities. Only the reward $r_{v(t)}(t)$ of the chosen arm $v(t)$, is then revealed to the policy-designer. We will use $r_{v(t)}$ in place of $r_{v(t)}(t)$ for notational convenience. 

%The objective is to learn a \textit{good} mapping from the space of contexts $\mathcal{X}$ to the space of arms $[K] = \{1,2,...,K\}$ in terms of expected reward and also to ensure that most of the arms are chosen according to this mapping as time progresses. The problem has been modeled in the literature~\cite{langford2008epoch,agarwal2014taming, dudik2011efficient} as stochastic contextual bandits with \textit{experts}. 


\begin{figure}[h]
	\centering
	\includegraphics[width=0.75\linewidth]{illustrate}
	\caption{\small Bayesian Network denoting the joint distribution of the random variables at a given time-step, under our contextual bandit setting. $X$ denotes the context, $V$ denotes the chosen arm, while $Y$ denotes the reward from the chosen arm that also depends on the context observed. The distribution of the reward given the chosen arm and the context, and the marginal of the context remain fixed over all time slots. However, the conditional distribution of the chosen arm given the context is dependent on the stochastic expert at that time-step. }
	\label{fig:illustrate}
\end{figure}

{\bf Stochastic Experts: } %In the experts setting the objective is to compete against $N$ experts/functions $\Pi = \{\pi_1,\cdots, \pi_N \}$ where each $\pi_i$ is a deterministic function mapping $\mathcal{X} \rightarrow [K]$. In the literature, the class of experts has been used as an abstraction for classifying functions that can take in the context as an input and produce the best arm as an output. However, well calibrated classifiers trained using supervised learning techniques are capable of supplying a confidence score for each arm which signifies the likelihood of the classifier choosing that arm as the best arm. Motivated by this observation, 
We consider a class of stochastic experts $\Pi = \{\pi_1,\cdots, \pi_N \}$, where each $\pi_i$ is a conditional probability distribution $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context. We will use the shorthand $\pi_i(V \vert X)$ to denote the conditional distribution corresponding to expert $i$, for notational convenience. The observation model at each time step $t$ is as follows: {\it (i)} A context $x_t$ is observed. {\it (ii)} The policy-designer chooses a stochastic expert $\pi_{k(t)} \in \Pi$. An arm $v(t)$ is drawn from the probability distribution $\pi_{k(t)}(V \vert x_t)$, by the policy-designer.  {\it (iv)} The stochastic reward $y_t = r_{v(t)}$ is revealed. 

The joint distribution of the random variables $X,V,Y$ denoting the context, arm chosen and reward observed respectively at time $t$, can be modeled by the Bayesian Network shown in Fig.~\ref{fig:illustrate}. The joint distribution factorizes as follows, 

\begin{align}
\label{eq:joint}
p(x,v,y) = p(y \vert v,x ) p(v \vert x)p(x) 
\end{align}
where $p(y \vert v,x )$ (the reward distribution given the arm and the context), and $p(x)$ (marginal distribution of the context) is determined by the nature's distribution and are fixed for all time-steps $t = 1,2,...,T$. On the other hand $p(v \vert x)$ (distribution of the arm chosen given the context) depends on the expert selected at each round. At time $t$, $p(v \vert x) = \pi_{k(t)}(v \vert x)$ that is the conditional distribution encoded by the stochastic expert chosen at time $t$. Now we are at a position to define the objective of the problem. 

{\bf Regret: } The objective in our contextual bandit problem is to perform as well as the best expert in the class of experts. We will define $p_k(x,v,y) \triangleq p(y \vert v,x ) \pi_k(v \vert x)p(x)$ as the distribution of the corresponding random variables when the expert chosen is $\pi_k \in \Pi$. The expected reward of expert $k$ is now denoted by,
 $\mu_k = \EE_{p_k(x,v,y)}[Y],$ where $\EE_{p(.)}$ denotes expectation with respect to distribution $p(.)$. The best expert is given by $k^* = \argmax_{k \in [N]} \mu_k$. The objective is to minimize the \textit{regret} till time $T$, which is defined as $R(T) = \sum_{t = 1}^{T} \left(\mu^* - \mu_{k(t)} \right)$, where $\mu^* = \mu_{k^*}$. Note that this is analogous to the regret definition for the deterministic \textit{expert} setting~\cite{langford2008epoch}. Let us define $\Delta_{k} \triangleq \mu^* - \mu_k$ as the optimality gap in terms of expected reward, for expert $k$. Let $\pmb{\mu} \triangleq \{\mu_1,...,\mu_N \}$.  Now we will define some divergence metrics that will be important in describing our algorithms and theoretical guarantees. 
 
% \begin{align}
% \label{eq:regret}
% R(T) = \sum_{t = 1}^{T} \left(\mu^* - \mu_{k(t)} \right),
% \end{align}
 
 
 \subsection{Divergence Metrics}
 \label{sec:divergence}
 In this section, we will define some general divergence metrics which will be important in our analysis. Before we proceed, we will define a general class of information theoretic quantities, $f$-divergences. 
 
 \begin{definition}
 	Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$.
 	For two joint distributions $p_{X,Y}(x,y)$ and $q_{X,Y}(x,y)$ (and the
 	associated  conditionals), the conditional $f$-divergence $D_{f}(p_{X
 		\vert Y} \Vert q_{X \vert Y})$ is given by: 
 	
 	$D_{f}(p_{X \vert Y} \Vert q_{X \vert Y}) = \EE_{q_{X,Y}} \left[f \left( \frac{p_{X \vert Y}(X \vert Y)}{q_{X \vert Y}(X \vert Y)} \right)\right].$

 \end{definition}
 
 Recall that $\pi_i$ is a conditional distribution of $V$ given $X$. Thus, $D_f(\pi_i \Vert
 \pi_j)$ is the conditional $f$-divergence between the conditional distributions $\pi_i$ and $\pi_j.$ Note that in this definition the marginal distribution of $X$ is the marginal of $X$ given by nature's inherent distribution over the contexts. In this work we will be concerned with two specific $f$-divergence metrics that are defined as follows. 
 
 \begin{definition}
 	\label{def:mij}
 	($M_{ij}$ measure)  Consider the function $f_1(x) = x \exp (x-1) -
 	1$. We define the following log-divergence measure:  $M_{ij} = 1 +
 	\log (1 + D_{f_1} (\pi_i \lVert \pi_j)),$ $\forall i,j
 	\in [N].$ 
 \end{definition}
 
 The $M_{ij}$-measures will be crucial in analyzing one of our estimators (clipped estimator) defined in Section~\ref{sec:estimators}. 
 
 \begin{definition}
 	\label{def:sij}
 	($\sigma_{ij}$ measure) $D_{f_2} (\pi_i \Vert \pi_j)$ is known as the chi-square divergence between the respective conditional distributions, where $f_2(x) = x^2 - 1$. Let $\sigma^2_{ij} = 1 + D_{f_2} (\pi_i \Vert \pi_j)$. 
 \end{definition}

The $\sigma_{ij}$-measures are important in analyzing our second estimator (median of means) defined in Section~\ref{sec:estimators}.


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Modern machine learning applications like recommendation engines~\cite{li2011scene,sen2016contextual,bouneffouf2012contextual,li2010contextual}, computational advertising~\cite{tang2013automatic,bottou2013counterfactual}, A/B testing in medicine~\cite{tekin2015discover,tekin2016adaptive} are inherently online. In these settings the task is to take sequential decisions that are not only profitable but also enable the system to learn better in future. For instance in a computational advertising system, the task is to sequentially place advertisements on users' webpages with the dual objective of learning the preferences of the users and increasing the click-through rate on the fly. A key attribute of these systems is the well-known \textit{exploration} (searching the space of possible decisions for better learning) and \textit{exploitation} (taking decisions that are more profitable) trade-off. A principled method to capture this trade-off is the study of multi-armed bandit problems~\cite{bubeck2012regret}.

Bandit problems have been studied for several decades. The classic $K$-armed bandit problem dates back to~\cite{lai1985asymptotically}. In the stochastic setting, one is faced with the choice of pulling one arm during each time-slot among $K$ arms, where the $k$-th arm has mean reward $\mu_k$. The task is to accumulate a total reward as close as possible to a genie strategy that has prior knowledge of arm statistics and always selects the optimal arm in each time-slot. The expected difference between the rewards collected by the genie strategy and the online strategy is defined as the regret. The expected regret till time $T$, of the state of the art algorithms~\cite{bubeck2012regret,auer2010ucb,agrawal2012analysis,auer2002using} scales as $O((K/\Delta) \log T )$ when there is a constant gap in mean reward of at least $\Delta$ between the best arm and the rest.

In the presence of side information, a popular model is that of contextual bandits. In the stochastic setting, it is assumed that at each time-step nature draws $(x,r_1,...,r_K)$ from a fixed but unknown distribution. Here, $x \in \mathcal{X}$ represents the context vector, while $r_1,...,r_K$ are the rewards of the $K$-arms~\cite{langford2008epoch}. The context $x$ is revealed to the policy-designer, after which she decides to choose an arm $a \in \{1,2,...,K \}$. Then, the reward $r_a$ is revealed to the policy-designer. In the computational advertising example, the context can be thought of as the browsing history, age, gender etc. of an user arriving in the system, while $r_1,...,r_K$ are generated according to the probability of the user clicking on each of the $K$ advertisements. The task here is to learn a \textit{good} mapping from the space of contexts $\mathcal{X}$ to the space of arms $[K] = \{1,2,...,K\}$ such that when the decisions are taken according to that mapping, the mean reward observed is high.  

The above problem is usually modeled in the literature as stochastic contextual bandits with \textit{experts}~\cite{agarwal2014taming,dudik2011efficient,langford2008epoch}. The task is to compete against the best \textit{expert} in a class of experts $\Pi = \{\pi_1,...,\pi_N\}$, where each expert $\pi \in \Pi$ is a function mapping $\mathcal{X} \rightarrow [K]$. The mean reward of an expert $\pi$ is defined as $ \EE \left[ r_{\pi(X)} \right]$, where $X$ is the random variable denoting the context and the expectation is taken over the unknown distribution over $(x,r_1,...,r_K)$. The best expert is naturally defined as the expert with the highest mean reward. The expected difference in rewards of a genie policy that always chooses the best expert and the online algorithm employed by the policy-designer is defined as the regret. This problem has been well-studied in the literature, where a popular approach is to reduce the contextual bandit problem to supervised learning techniques through $\argmin$-oracles~\cite{beygelzimer2009offset}. This leads to powerful algorithms with instance-independent regret bounds of $\mathcal{O} \left(\sqrt{KT\mathrm{polylog}(N)} \right)$ at time $T$~\cite{agarwal2014taming,dudik2011efficient}. In this setting, the class of experts $\Pi$ can be thought of as a class of classifying functions that classify each context into one of the $K$ arms. 

We consider the problem of contextual bandits with \textit{stochastic experts}. Our problem setting is closely related to the traditional experts setting in stochastic bandits~\cite{agarwal2014taming,dudik2011efficient}, with a subtle distinction. We assume access to a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, which are \textit{not deterministic}. %functions mapping $\mathcal{X} \rightarrow [K]$. 
Instead, each expert $\pi \in \Pi$, is a conditional probability distribution over the arms given a context. For, an expert $\pi \in \Pi$ the conditional distribution is denoted by $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context.  One key motivation is that this allows us to derive regret bounds in terms of \textit{closeness} of these soft experts quantified by divergence measures, rather than in terms of the total number of arms $K$. Another motivation is that the cost-sensitive classification oracles used to generate deterministic experts in a practical algorithm (in the traditional experts setting~\cite{agarwal2014taming}), can be calibrated using well-known techniques~\cite{cohen2004properties}, such that they can provide reliable confidence scores for each arm. These confidence scores are precisely a probability distribution over the arms, that encodes soft belief of an expert about the best arm, given a context.

As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$. We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem. We prove \textit{instance-dependent} regret guarantees that scale as $\mathcal{O} \left(\mathcal{C} \left(N,\Delta\right) \log T\right)$, where $\mathcal{C} \left(N,\Delta\right)$  is an instance dependent term. We show that under some assumptions the term $\mathcal{C} \left(N,\Delta\right)$ scales as $\mathcal{O}(\log N/ \Delta)$, where $\Delta$ is the gap in mean reward of the best expert from second best. In the next section, we list the main contributions of this paper. 

%It should be noted that modern classifiers can be calibrated using well-known techniques~\cite{cohen2004properties}, such that they can provide reliable confidence scores for each class. Motivated by this observation, we model the contextual bandit problem with stochastic experts. In this setting, we have a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, where each $\pi_i$ is a conditional probability distribution $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context. As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$. We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem. We prove \textit{instance-dependent} regret guarantees that scale as $\mathcal{O} \left(\mathcal{C} \left(N,\Delta\right) \log T\right)$, where $\mathcal{C} \left(N,\Delta\right)$  is an instance dependent term. We show that under some assumptions the term $\mathcal{C} \left(N,\Delta\right)$ scales as $\mathcal{O}(\log N/ \Delta)$, where $\Delta$ is the gap in mean reward of the best expert from second best. In the next section, we list the main contributions of this paper. 

\subsection{Main Contributions}
The contributions of this paper are three-folds:

{\bf $(i)$ (Instance Dependent Regret Bounds):}  We propose the contextual bandits with stochastic experts problem. We design two UCB based algorithms for this problem, based on two different importance sampling based estimators for estimating the mean of each expert. The key idea behind these estimators is that samples collected by deploying an expert can be used to estimate the mean reward under another expert. This \textit{information leakage} helps us in achieving regret guarantees that scale sub-linearly in $N$, the number of experts. We analyze UCB based algorithms under two such estimators, the clipped estimator~\eqref{eq:est1} (introduced in~\cite{pmlr-v70-sen17a}) and the median of means estimator~\eqref{eq:est2} (proposed in this paper). The information leakage between any two experts in the first estimator is governed by a pairwise log-divergence measure (Def.~\ref{def:mij}). For the second estimator, chi-square divergence (Def.~\ref{def:sij}) characterizes it.

We show that the regret of our UCB algorithm based on these two estimators scales as \footnote{Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. Here, we only mention the Corollaries of our approach, that are easy to state.}:
\[ \mathcal{O}\left(  \frac{\lambda(\pmb{\mu}) \mathcal{M}}{\Delta}  \log T  \right) \]
Here, $\mathcal{M}$ is related to the largest pairwise divergence values under the two divergence measures used. $\Delta$ is the gap between the mean rewards of the optimal expert and the second best. $\lambda(\pmb{\mu})$ is a parameter that only depends on the gaps between mean rewards of the optimum experts and various sub-optimal ones. It is a normalized sum of difference in squares of the gaps of adjacent sub-optimal experts ordered by their gaps. Under the assumption that the suboptimal gaps (except that of the second best arm) are uniformly distributed in a bounded interval, we can show that the parameter $\lambda(\pmb{\mu})$ is $O(\log N)$. We define this parameter explicitly in Section \ref{sec:results} for all problem instances.

 For the clipped estimator we show that $\mathcal{M}= M^2 \log^2 (1/\Delta)$ where $M$ is the largest pairwise log-divergence associated with the clipped estimator. For the median of means estimator,  $\mathcal{M}= \sigma^2 $ where $\sigma^2$ is the largest pairwise chi-squared divergence. %Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. 
 
 Naively treating each expert as an arm would lead to a regret scaling of $\mathcal{O}(N \log T/ \Delta)$. However, this ignores information leakage. Existing instance-independent bounds for contextual bandits scale as $\sqrt{KT \mathrm{poly} \log(N) }$. Our problem dependent bounds have a near optimal dependence on $\Delta$ and does not depend on $K$, the numbers of arms. However, it depends on the divergence measure associated with the information leakage in the problem ($M$ or $\sigma$ parameters). Besides our analysis, we empirically show that this divergence based approach rivals or performs better than very efficient heuristics for contextual bandits (like bagging etc.) on real-world data sets.

%The exact dependence in presented as Theorem~\ref{thm:r1}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{M^2 \log^2 (1/\Delta)\log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\Delta$ is the minimum gap in expected reward of the best expert and the rest, and $M$ is a divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{M}$ is $\mathcal{O} \left( \frac{M^2 \log ^2 (1/\Delta) }{\Delta^2}\right)$, thus independent of $N$. 
%
%Similarly, the regret of the algorithm based on the median of means estimator~\eqref{eq:est2} scales $\mathcal{O}\left(\mathcal{S} \log T \right)$, where $\mathcal{S}$ is an instance dependent term that depends on the mean reward gaps between the experts and the amount of information leakage between the experts. The exact dependence in presented as Theorem~\ref{thm:r2}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{\sigma^2 \log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\sigma$ is another divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{S}$ is $\mathcal{O} \left( \frac{\sigma^2 }{\Delta^2}\right)$, thus independent of $N$.


{\bf $(ii)$ (Importance Sampling based Estimators):}
As mentioned before, the key components in our UCB based algorithm are two estimators that can utilize the samples collected under all the experts, in order to estimate the mean reward under any given expert. Both of these estimators are based on importance sampling techniques. %, which uses the fact that the samples collected under one expert can be reweighed by an importance ratio, to estimate the mean under another expert. 
The first estimator that we use is the clipped estimator~\eqref{eq:est1}, which was introduced in~\cite{pmlr-v70-sen17a}. However, we modify the clipper level adaptively over the course of our UCB algorithm, in order to achieve our regret guarantees. 

We also propose a novel median of means~\eqref{eq:est2} based importance sampling estimator for estimating the mean under all experts, utilizing this information leakage among experts. To the best of our knowledge, importance sampling has not been used in conjunction with the median of means technique in the literature before. We provide novel confidence guarantees for this estimator which depends on chi-square divergence between the conditional distributions under the various experts. This may be of independent interest. 

{\bf $(iii)$ (Empirical Validation):} We empirically validate our algorithm on three real world data-sets~\cite{frey1991letter,fehrman2017five,stream} against other state of the art contextual bandit algorithms~\cite{langford2008epoch,agarwal2014taming} implemented in Vowpal Wabbit~\cite{wabbit}. In our implementation, we use online training of cost-sensitive classification oracles~\cite{beygelzimer2009offset} to generate the class of stochastic experts. We show that our algorithms have better regret performance on these data-sets compared to the other algorithms. 

  

==> introductionv2.tex <==
\section{Introduction}
\label{sec:intro}
Modern machine learning applications like recommendation engines~\cite{li2011scene,sen2016contextual,bouneffouf2012contextual,li2010contextual}, computational advertising~\cite{tang2013automatic,bottou2013counterfactual}, A/B testing in medicine~\cite{tekin2015discover,tekin2016adaptive} are inherently online. In these settings the task is to take sequential decisions that are not only profitable but also enable the system to learn better in future. For instance in a computational advertising system, the task is to sequentially place advertisements on users' webpages with the dual objective of learning the preferences of the users and increasing the click-through rate on the fly. A key attribute of these systems is the well-known \textit{exploration} (searching the space of possible decisions for better learning) and \textit{exploitation} (taking decisions that are more profitable) trade-off. A principled method to capture this trade-off is the study of multi-armed bandit problems~\cite{bubeck2012regret}.

Bandit problems have been studied for several decades. The classic $K$-armed bandit problem dates back to~\cite{lai1985asymptotically}. In the stochastic setting, one is faced with the choice of pulling one arm during each time-slot among $K$ arms, where the $k$-th arm has mean reward $\mu_k$. The task is to accumulate a total reward as close as possible to a genie strategy that has prior knowledge of arm statistics and always selects the optimal arm in each time-slot. The expected difference between the rewards collected by the genie strategy and the online strategy is defined as the regret. The expected regret till time $T$, of the state of the art algorithms~\cite{bubeck2012regret,auer2010ucb,agrawal2012analysis,auer2002using} scales as $O((K/\Delta) \log T )$ when there is a constant gap in mean reward of at least $\Delta$ between the best arm and the rest.

Additional side information can be incorporated in this setting through the framework of contextual bandits. In the stochastic setting, it is assumed that at each time-step nature draws $(x,r_1,...,r_K)$ from a fixed but unknown distribution. Here, $x \in \mathcal{X}$ represents the context vector, while $r_1,...,r_K$ are the rewards of the $K$-arms~\cite{langford2008epoch}. The context $x$ is revealed to the policy-designer, after which she decides to choose an arm $a \in \{1,2,...,K \}$. Then, the reward $r_a$ is revealed to the policy-designer. In the computational advertising example, the context can be thought of as the browsing history, age, gender etc. of an user arriving in the system, while $r_1,...,r_K$ are generated according to the probability of the user clicking on each of the $K$ advertisements. The task here is to learn a \textit{good} mapping from the space of contexts $\mathcal{X}$ to the space of arms $[K] = \{1,2,...,K\}$ such that when the decisions are taken according to that mapping, the mean reward observed is high.

A popular model in the stochastic contextual bandits literature is the \textit{experts} setting~\cite{agarwal2014taming,dudik2011efficient,langford2008epoch}. The task is to compete against the best \textit{expert} in a class of experts $\Pi = \{\pi_1,...,\pi_N\}$, where each expert $\pi \in \Pi$ is a function mapping $\mathcal{X} \rightarrow [K]$. The mean reward of an expert $\pi$ is defined as $ \EE \left[ r_{\pi(X)} \right]$, where $X$ is the random variable denoting the context and the expectation is taken over the unknown distribution over $(x,r_1,...,r_K)$. The best expert is naturally defined as the expert with the highest mean reward. The expected difference in rewards of a genie policy that always chooses the best expert and the online algorithm employed by the policy-designer is defined as the regret. This problem has been well-studied in the literature, where a popular approach is to reduce the contextual bandit problem to supervised learning techniques through $\argmin$-oracles~\cite{beygelzimer2009offset}. This leads to powerful algorithms with instance-independent regret bounds of $\mathcal{O} \left(\sqrt{KT\mathrm{polylog}(N)} \right)$ at time $T$~\cite{agarwal2014taming,dudik2011efficient}. In this setting, the class of experts $\Pi$ can be thought of as a class of classifying functions that classify each context into one of the $K$ arms. 

We consider the problem of contextual bandits with \textit{stochastic experts}. Our problem setting is closely related to the traditional experts setting in stochastic bandits~\cite{agarwal2014taming,dudik2011efficient}, with a subtle distinction. We assume access to a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, which are \textit{not deterministic}. %functions mapping $\mathcal{X} \rightarrow [K]$.
Instead, each expert $\pi \in \Pi$, is a conditional probability distribution over the arms given a context. For, an expert $\pi \in \Pi$ the conditional distribution is denoted by $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context.  They key motivation is that the cost-sensitive classification oracles used to generate deterministic experts in a practical algorithm (in the traditional experts setting~\cite{agarwal2014taming}) can be calibrated using well-known techniques~\cite{cohen2004properties}, such that they can provide reliable confidence scores for each arm. These confidence scores are precisely a probability distribution over the arms, and encodes a soft belief of an expert about the best arm given a context. An additional benefit is that this setting allows us to derive regret bounds in terms of \textit{closeness} of these soft experts quantified by divergence measures, rather than in terms of the total number of arms $K$.  As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$.

We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem. We prove \textit{instance-dependent} regret guarantees that scale as $\mathcal{O} \left(\mathcal{C} \left(N,\Delta\right) \log T\right)$, where $\mathcal{C} \left(N,\Delta\right)$  is an instance dependent term. We show that under some assumptions the term $\mathcal{C} \left(N,\Delta\right)$ scales as $\mathcal{O}(\log N/ \Delta)$, where $\Delta$ is the gap in mean reward of the best expert from second best. In the next section, we list the main contributions of this paper. 

%It should be noted that modern classifiers can be calibrated using well-known techniques~\cite{cohen2004properties}, such that they can provide reliable confidence scores for each class. Motivated by this observation, we model the contextual bandit problem with stochastic experts. In this setting, we have a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, where each $\pi_i$ is a conditional probability distribution $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context. As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$. We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem. We prove \textit{instance-dependent} regret guarantees that scale as $\mathcal{O} \left(\mathcal{C} \left(N,\Delta\right) \log T\right)$, where $\mathcal{C} \left(N,\Delta\right)$  is an instance dependent term. We show that under some assumptions the term $\mathcal{C} \left(N,\Delta\right)$ scales as $\mathcal{O}(\log N/ \Delta)$, where $\Delta$ is the gap in mean reward of the best expert from second best. In the next section, we list the main contributions of this paper. 

\subsection{Main Contributions}
The contributions of this paper are three-folds:

{\bf $(i)$ (Importance Sampling based Estimators):}
The key components in our approach are two importance sampling based estimators for the mean rewards under all the experts. Both these estimators are based on the observation that samples collected under one expert can be reweighed by likelihood/importance ratios and averaged to provide an estimate for the mean reward under another expert. This sharing of information is termed as \textit{information leakage} and has been utilized before under various settings~\cite{lattimore2016causal,pmlr-v70-sen17a,bottou2013counterfactual}. The first estimator that we use is an adaptive variant of the well-known clipping technique, which was proposed in~\cite{pmlr-v70-sen17a}. The estimator is presented in Eq.~\eqref{eq:est1}. However, we carefully adapt the clipping threshold in an online manner, in order to achieve regret guarantees. 

We also propose an importance sampling variant of the classical median of means estimator (see ~\cite{lugosi2017sub,bubeck2013bandits}). This estimator is also designed to utilize the samples collected under all experts together to estimate the mean reward under any given expert. We define the estimator in Eq.~\eqref{eq:est2}. To the best of our knowledge, importance sampling has not been used in conjunction with the median of means technique in the literature before. We provide novel confidence guarantees for this estimator which depends on chi-square divergences between the conditional distributions under the various experts. This may be of independent interest. 

{\bf $(ii)$ (Instance Dependent Regret Bounds):}  We propose the contextual bandits with stochastic experts problem. We design two UCB based algorithms for this problem, based on the two importance sampling based estimators mentioned above. We show that utilizing the \textit{information leakage} between the experts leads to regret guarantees that scale sub-linearly in $N$, the number of experts. The information leakage between any two experts in the first estimator is governed by a pairwise log-divergence measure (Def.~\ref{def:mij}). For the second estimator, chi-square divergences (Def.~\ref{def:sij}) characterizes the leakage.

We show that the regret of our UCB algorithm based on these two estimators scales as \footnote{Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. Here, we only mention the Corollaries of our approach, that are easy to state.}: $ \mathcal{O}\left(  \frac{\lambda(\pmb{\mu}) \mathcal{M}}{\Delta}  \log T  \right)$.

Here, $\mathcal{M}$ is related to the largest pairwise divergence values under the two divergence measures used. $\Delta$ is the gap between the mean rewards of the optimal expert and the second best. $\lambda(\pmb{\mu})$ is a parameter that only depends on the gaps between mean rewards of the optimum experts and various sub-optimal ones. It is a normalized sum of difference in squares of the gaps of adjacent sub-optimal experts ordered by their gaps. Under the assumption that the suboptimal gaps (except that of the second best arm) are uniformly distributed in a bounded interval, we can show that the parameter $\lambda(\pmb{\mu})$ is $O(\log N)$ in expectation. We define this parameter explicitly in Section \ref{sec:results}.

 For the clipped estimator we show that $\mathcal{M}= M^2 \log^2 (1/\Delta)$ where $M$ is the largest pairwise log-divergence associated with the clipped estimator. For the median of means estimator,  $\mathcal{M}= \sigma^2 $ where $\sigma^2$ is the largest pairwise chi-squared divergence. %Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. 
 
 Naively treating each expert as an arm would lead to a regret scaling of $\mathcal{O}(N \log T/ \Delta)$. However, this ignores information leakage. Existing instance-independent bounds for contextual bandits scale as $\sqrt{KT \mathrm{poly} \log(N) }$~\cite{agarwal2014taming}. Our problem dependent bounds have a near optimal dependence on $\Delta$ and does not depend on $K$, the numbers of arms. However, it depends on the divergence measure associated with the information leakage in the problem ($M$ or $\sigma$ parameters). Besides our analysis, we empirically show that this divergence based approach rivals or performs better than very efficient heuristics for contextual bandits (like bagging etc.) on real-world data sets.

%The exact dependence in presented as Theorem~\ref{thm:r1}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{M^2 \log^2 (1/\Delta)\log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\Delta$ is the minimum gap in expected reward of the best expert and the rest, and $M$ is a divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{M}$ is $\mathcal{O} \left( \frac{M^2 \log ^2 (1/\Delta) }{\Delta^2}\right)$, thus independent of $N$. 
%
%Similarly, the regret of the algorithm based on the median of means estimator~\eqref{eq:est2} scales $\mathcal{O}\left(\mathcal{S} \log T \right)$, where $\mathcal{S}$ is an instance dependent term that depends on the mean reward gaps between the experts and the amount of information leakage between the experts. The exact dependence in presented as Theorem~\ref{thm:r2}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{\sigma^2 \log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\sigma$ is another divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{S}$ is $\mathcal{O} \left( \frac{\sigma^2 }{\Delta^2}\right)$, thus independent of $N$.


{\bf $(iii)$ (Empirical Validation):} We empirically validate our algorithm on three real world data-sets~\cite{frey1991letter,fehrman2017five,stream} against other state of the art contextual bandit algorithms~\cite{langford2008epoch,agarwal2014taming} implemented in Vowpal Wabbit~\cite{wabbit}. In our implementation, we use online training of cost-sensitive classification oracles~\cite{beygelzimer2009offset} to generate the class of stochastic experts. We show that our algorithms have better regret performance on these data-sets compared to the other algorithms. 

  

==> introductionv3.tex <==
\section{Introduction}
\label{sec:intro}
Modern machine learning applications like recommendation engines~\cite{li2011scene,bouneffouf2012contextual,li2010contextual}, computational advertising~\cite{tang2013automatic,bottou2013counterfactual}, A/B testing in medicine~\cite{tekin2015discover,tekin2016adaptive} are inherently online. In these settings the task is to take sequential decisions that are not only profitable but also enable the system to learn better in future. For instance in a computational advertising system, the task is to sequentially place advertisements on users' webpages with the dual objective of learning the preferences of the users and increasing the click-through rate on the fly. A key attribute of these systems is the well-known \textit{exploration} (searching the space of possible decisions for better learning) and \textit{exploitation} (taking decisions that are more profitable) trade-off. A principled method to capture this trade-off is the study of multi-armed bandit problems~\cite{bubeck2012regret}.

Bandit problems have been studied for several decades. The classic $K$-armed bandit problem dates back to~\cite{lai1985asymptotically}. In the stochastic setting, one is faced with the choice of pulling one arm during each time-slot among $K$ arms, where the $k$-th arm has mean reward $\mu_k$. The task is to accumulate a total reward as close as possible to a genie strategy that has prior knowledge of arm statistics and always selects the optimal arm in each time-slot. The expected difference between the rewards collected by the genie strategy and the online strategy is defined as the regret. The expected regret till time $T$, of the state of the art algorithms~\cite{bubeck2012regret,auer2010ucb,agrawal2012analysis,auer2002using} scales as $O((K/\Delta) \log T )$ when there is a constant gap in mean reward of at least $\Delta$ between the best arm and the rest.

Additional side information can be incorporated in this setting through the framework of contextual bandits. In the stochastic setting, it is assumed that at each time-step nature draws $(x,r_1,...,r_K)$ from a fixed but unknown distribution. Here, $x \in \mathcal{X}$ represents the context vector, while $r_1,...,r_K$ are the rewards of the $K$-arms~\cite{langford2008epoch}. The context $x$ is revealed to the policy-designer, after which she decides to choose an arm $a \in \{1,2,...,K \}$. Then, the reward $r_a$ is revealed to the policy-designer. In the computational advertising example, the context can be thought of as the browsing history, age, gender etc. of an user arriving in the system, while $r_1,...,r_K$ are generated according to the probability of the user clicking on each of the $K$ advertisements. The task here is to learn a \textit{good} mapping from the space of contexts $\mathcal{X}$ to the space of arms $[K] = \{1,2,...,K\}$ such that when the decisions are taken according to that mapping, the mean reward observed is high.

A popular model in the stochastic contextual bandits literature is the \textit{experts} setting~\cite{agarwal2014taming,dudik2011efficient,langford2008epoch}. The task is to compete against the best \textit{expert} in a class of experts $\Pi = \{\pi_1,...,\pi_N\}$, where each expert $\pi \in \Pi$ is a function mapping $\mathcal{X} \rightarrow [K]$. The mean reward of an expert $\pi$ is defined as $ \EE \left[ r_{\pi(X)} \right]$, where $X$ is the random variable denoting the context and the expectation is taken over the unknown distribution over $(x,r_1,...,r_K)$. The best expert is naturally defined as the expert with the highest mean reward. The expected difference in rewards of a genie policy that always chooses the best expert and the online algorithm employed by the policy-designer is defined as the regret. This problem has been well-studied in the literature, where a popular approach is to reduce the contextual bandit problem to supervised learning techniques through $\argmin$-oracles~\cite{beygelzimer2009offset}. This leads to powerful algorithms with instance-independent regret bounds of $\mathcal{O} \left(\sqrt{KT\mathrm{polylog}(N)} \right)$ at time $T$~\cite{agarwal2014taming,dudik2011efficient}.  

In practice the class of experts are generated online by training cost-sensitive classification oracles~\cite{agarwal2014taming,dudik2011efficient}. The resulting classifiers/oracles trained can provide reliable confidence scores given a new context, especially if they are well-calibrated~\cite{cohen2004properties}. These confidence scores are nothing but a $K$-dimensional probability vector, where the $k^{th}$ entry is the probability of the classifier/oracle choosing the $k^{th}$ arm as the best, given a context. Motivated by this, we propose a variation of the traditional experts setting, which we term contextual bandits with \textit{stochastic experts.} We assume access to a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, which are \textit{not deterministic}. Instead, each expert $\pi \in \Pi$, is a conditional probability distribution over the arms given a context. For, an expert $\pi \in \Pi$ the conditional distribution is denoted by $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context.  An additional benefit is that this setting allows us to derive regret bounds in terms of \textit{closeness} of these soft experts quantified by divergence measures, rather than in terms of the total number of arms $K$.  

As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$. We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem, that employ two importance sampling based estimators for the mean rewards under various experts. We prove \textit{instance-dependent} regret guarantees for our algorithm. The main contributions of this paper are listed in the next Section. 


%that scale as $\mathcal{O} \left(\lambda(\pmb{\mu})\mathcal{M}\log T/ \Delta\right)$, where $\Delta$ is the gap in mean reward of the best expert from second best and $\mathcal{M}$ is a divergence term that measures the closeness between the experts.  We show that the term $\lambda(\pmb{\mu})$ which only depends on the relative mean reward gaps between that experts, can scale as $O(\log N)$ under some assumptions.  

%It should be noted that modern classifiers can be calibrated using well-known techniques~\cite{cohen2004properties}, such that they can provide reliable confidence scores for each class. Motivated by this observation, we model the contextual bandit problem with stochastic experts. In this setting, we have a class of \textit{stochastic experts} $\Pi = \{\pi_1,...,\pi_N\}$, where each $\pi_i$ is a conditional probability distribution $\pi_{V \vert X}(v \vert x)$ where $V \in [K]$ is the random variable denoting the arm chosen and $X$ is the context. As before, the task is to compete against the expert in the class with the highest mean reward. The expected reward of a stochastic expert $\pi$ is defined as $\EE_{X,V \sim \pi(V \vert X)} \left[ r_{V}\right]$, i.e the mean reward observed when the arm is drawn from the conditional distribution $\pi(V \vert X)$. We propose upper-confidence (UCB) style algorithms for the contextual bandits with stochastic experts problem. We prove \textit{instance-dependent} regret guarantees that scale as $\mathcal{O} \left(\mathcal{C} \left(N,\Delta\right) \log T\right)$, where $\mathcal{C} \left(N,\Delta\right)$  is an instance dependent term. We show that under some assumptions the term $\mathcal{C} \left(N,\Delta\right)$ scales as $\mathcal{O}(\log N/ \Delta)$, where $\Delta$ is the gap in mean reward of the best expert from second best. In the next section, we list the main contributions of this paper. 

\subsection{Main Contributions}
The contributions of this paper are three-folds:

{\bf $(i)$ (Importance Sampling based Estimators):}
The key components in our approach are two importance sampling based estimators for the mean rewards under all the experts. Both these estimators are based on the observation that samples collected under one expert can be reweighted by likelihood/importance ratios and averaged to provide an estimate for the mean reward under another expert. This sharing of information is termed as \textit{information leakage} and has been utilized before under various settings~\cite{lattimore2016causal,pmlr-v70-sen17a,bottou2013counterfactual}. The first estimator that we use is an adaptive variant of the well-known clipping technique, which was proposed in~\cite{pmlr-v70-sen17a}. The estimator is presented in Eq.~\eqref{eq:est1}. However, we carefully adapt the clipping threshold in an online manner, in order to achieve regret guarantees. 

We also propose an importance sampling variant of the classical median of means estimator (see ~\cite{lugosi2017sub,bubeck2013bandits}). This estimator is also designed to utilize the samples collected under all experts together to estimate the mean reward under any given expert. We define the estimator in Eq.~\eqref{eq:est2}. To the best of our knowledge, importance sampling has not been used in conjunction with the median of means technique in the literature before. We provide novel confidence guarantees for this estimator which depends on chi-square divergences between the conditional distributions under the various experts. This may be of independent interest. 

{\bf $(ii)$ (Instance Dependent Regret Bounds):}  We propose the contextual bandits with stochastic experts problem. We design two UCB based algorithms for this problem, based on the two importance sampling based estimators mentioned above. We show that utilizing the \textit{information leakage} between the experts leads to regret guarantees that scale sub-linearly in $N$, the number of experts. The information leakage between any two experts in the first estimator is governed by a pairwise log-divergence measure (Def.~\ref{def:mij}). For the second estimator, chi-square divergences (Def.~\ref{def:sij}) characterize the leakage.

We show that the regret of our UCB algorithm based on these two estimators scales as \footnote{Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. Here, we only mention the Corollaries of our approach, that are easy to state.}: $ \mathcal{O}\left(  \frac{\lambda(\pmb{\mu}) \mathcal{M}}{\Delta}  \log T  \right)$.

Here, $\mathcal{M}$ is related to the largest pairwise divergence values under the two divergence measures used. $\Delta$ is the gap between the mean rewards of the optimal expert and the second best. $\lambda(\pmb{\mu})$ is a parameter that only depends on the gaps between mean rewards of the optimum experts and various sub-optimal ones. It is a normalized sum of difference in squares of the gaps of adjacent sub-optimal experts ordered by their gaps. Under the assumption that the suboptimal gaps (except that of the second best arm) are uniformly distributed in a bounded interval, we can show that the parameter $\lambda(\pmb{\mu})$ is $O(\log N)$ in expectation. We define this parameter explicitly in Section \ref{sec:results}.

 For the clipped estimator we show that $\mathcal{M}= M^2 \log^2 (1/\Delta)$ where $M$ is the largest pairwise log-divergence associated with the clipped estimator. For the median of means estimator,  $\mathcal{M}= \sigma^2 $ where $\sigma^2$ is the largest pairwise chi-squared divergence. %Tighter regret bounds are derived in Theorems \ref{thm:r1} and \ref{thm:r2}. 
 
 Naively treating each expert as an arm would lead to a regret scaling of $\mathcal{O}(N \log T/ \Delta)$. However, this ignores information leakage. Existing instance-independent bounds for contextual bandits scale as $\sqrt{KT \mathrm{poly} \log(N) }$~\cite{agarwal2014taming}. Our problem dependent bounds have a near optimal dependence on $\Delta$ and does not depend on $K$, the numbers of arms. However, it depends on the divergence measure associated with the information leakage in the problem ($M$ or $\sigma$ parameters). Besides our analysis, we empirically show that this divergence based approach rivals or performs better than very efficient heuristics for contextual bandits (like bagging etc.) on real-world data sets.

%The exact dependence in presented as Theorem~\ref{thm:r1}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{M^2 \log^2 (1/\Delta)\log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\Delta$ is the minimum gap in expected reward of the best expert and the rest, and $M$ is a divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{M}$ is $\mathcal{O} \left( \frac{M^2 \log ^2 (1/\Delta) }{\Delta^2}\right)$, thus independent of $N$. 
%
%Similarly, the regret of the algorithm based on the median of means estimator~\eqref{eq:est2} scales $\mathcal{O}\left(\mathcal{S} \log T \right)$, where $\mathcal{S}$ is an instance dependent term that depends on the mean reward gaps between the experts and the amount of information leakage between the experts. The exact dependence in presented as Theorem~\ref{thm:r2}. We show that when the mean rewards of the experts are uniformly distributed then the regret scales as $\mathcal{O} \left( \frac{\sigma^2 \log T\log N }{\Delta}\right)$ in expectation, thus only scaling logarithmically in the number of experts. Here, $\sigma$ is another divergence term that quantifies the information leakage among the experts. Alternatively, we can also prove that the term $\mathcal{S}$ is $\mathcal{O} \left( \frac{\sigma^2 }{\Delta^2}\right)$, thus independent of $N$.


{\bf $(iii)$ (Empirical Validation):} We empirically validate our algorithm on three real world data-sets~\cite{frey1991letter,fehrman2017five,stream} against other state of the art contextual bandit algorithms~\cite{langford2008epoch,agarwal2014taming} implemented in Vowpal Wabbit~\cite{wabbit}. In our implementation, we use online training of cost-sensitive classification oracles~\cite{beygelzimer2009offset} to generate the class of stochastic experts. We show that our algorithms have better regret performance on these data-sets compared to the other algorithms. 

  

==> regret.tex <==
\section{Instance Dependent Terms}
\label{sec:regret}

In this section we devote our attention to the instance dependent terms in Theorems~\ref{thm:r1} and \ref{thm:r2}. We will first prove Corollary~\ref{cor:delta}. 

\begin{proof}[Proof of Corollary~\ref{cor:delta}]
	
	$(i)$ From Eq.~\eqref{eq:uselater} in the proof of Theorem~\ref{thm:r1}, it follows that the regret of Algorithm~\ref{alg:dUCB} under the clipped estimator is bounded by,
	\begin{align*}
	R(T) \leq \Delta_{(N)}T_{2} + \frac{\pi^2}{3} \left( \sum_{i} \Delta_{(i)}\right).
	\end{align*}
	Using the definition of $T_{2}$ in~\eqref{eq:uselater} we obtain the required result. 
	
	
	$(ii)$ From Eq.~\eqref{eq:uselater2} in the proof of Theorem~\ref{thm:r2}, it follows that the regret of Algorithm~\ref{alg:dUCB} under the median of means estimator is bounded by,
	\begin{align*}
	R(T) \leq \Delta_{(N)}T_{2} + \frac{\pi^2}{3} \left( \sum_{i} \Delta_{(i)}\right).
	\end{align*}
	Using the definition of $T_{2}$ in~\eqref{eq:uselater2} we obtain the required result. 
\end{proof}

Now we will work under the assumption that the means of the experts are generated according to the generative model in Lemma~\ref{lem:mu}. 

\begin{proof}[Proof of Lemma~\ref{lem:mu}]
We will prove the two parts of the lemma separately,

$(i)$ Now we work under the assumption that $\Delta_{(2)} > 1/T$. Therefore, going back to Lemma~\ref{lem:lbound}, we get that,
\begin{align*}
\PP(U_k(t) < \mu^*) \geq 1 - \frac{1}{t^2}
\end{align*}
when $t > \frac{144M^2\log^3T}{\Delta_k^2}$. Therefore, the chain leading to Eq.~\eqref{eq:uselater} follows with the new definition of $T_k = \frac{144M^2\log^3T}{\Delta_{(k)}^2}$. Hence, under this assumption the regret of Algorithm~\ref{alg:dUCB} under estimator~\eqref{eq:est1} is bounded as follows:
\begin{align*}
&R(T) \leq \frac{144M^2 \log^3 T}{\Delta_{(2)}} \left(1 + \sum_{k = 2}^{N-1} \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) \right) \\
&+ \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right). \numberthis \label{eq:r12}
\end{align*}
Now, we will assume that $\{\Delta_{(i)}\}$ for $i = 3,...,N$, are order statistics of $N-2$ i.i.d uniform r.vs over the interval $[\Delta_{(2)},1]$. 

	Note that by Jensen's we have the following:
\begin{align}
\label{eq:jensen}
1 - \EE \left[ \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right] \leq 1 - \EE \left[  \frac{\Delta_{(k)}}{\Delta_{(k+1)}} \right]^2. 
\end{align} 


Let $X = \Delta_{(k)}$ and $Y = \Delta_{(k+1)}$ for $k \geq 3$. The joint pdf of $X,Y$ is given by,

\begin{align*}
&f(x,y) = \frac{(N-2)!}{(k-1)!(N-3-k)!} \left(\frac{x - \Delta_{(2)}}{1 - \Delta_{(2)} } \right)^{k-1} \times \\
&\left(1 - \frac{y - \Delta_{(2)}}{1 - \Delta_{(2)} } \right)^{N -3 -k} \frac{1}{(1 - \Delta_{(2)} )^2}.
\end{align*}

Therefore, we have the following chain:
\begin{align*}
&\EE \left[ \frac{X}{Y}\right] = \int_{y = \Delta_{(2)} }^{1} \int_{x = \Delta_{(2)}}^{y} \frac{x}{y} \frac{(N-2)!}{(k-1)!(N-3-k)!} \times \\
&\left(\frac{x - \Delta_{(2)}}{1 - \Delta_{(2)} } \right)^{k-1} \left(1 - \frac{y - \Delta_{(2)}}{1 - \Delta_{(2)} } \right)^{N -3 -k} \frac{1}{(1 - \Delta_{(2)} )^2} dx dy \\
&= \int_{b = 0 }^{1} \int_{a = 0}^{b} \frac{(1 - \Delta_{(2)})a+ \Delta_{(2)}}{(1 - \Delta_{(2)})b+ \Delta_{(2)}} \frac{(N-2)!}{(k-1)!(N-3-k)!} \times \\
&\left(a \right)^{k-1} \left(1 -b \right)^{N -3 -k}  da db \\ 
&\geq \int_{b = 0 }^{1} \int_{a = 0}^{b} \frac{a}{b} \frac{(N-2)!}{(k-1)!(N-3-k)!} \left(a \right)^{k-1} \left(1 -b \right)^{N -3 -k}  da db \\
& = \frac{k}{k+1}. 
\end{align*}

Combining this with Eq~\eqref{eq:jensen} yields,
\begin{align*}
&\EE_{p_{\Delta}} \left[ \sum_{k = 2}^{N-1} \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) \right] \\
&\leq 1 + \sum_{k = 3}^{N-1} \left(1 -  \frac{k^2}{(k+1)^2} \right) \\
&= 1 + \sum_{k = 3}^{N-1} \left(\frac{2k+1}{(k+1)^2} \right) \\
&\leq 1 + \sum_{k = 3}^{N-1} \frac{2}{k+1} \numberthis \label{eq:deltabound}\\
&\leq 1 + 2\log N.
\end{align*}

Combining Eq.~\eqref{eq:deltabound} and Eq.~\eqref{eq:r12} yields the result. 

$(ii)$ Combining the regret guarantee in Theorem~\ref{thm:r2} with Eq.~\eqref{eq:deltabound} directly yields the desired result. 
\end{proof}



==> results.tex <==
\section{Theoretical Results}
\label{sec:results}
In this section we provide \textit{instance dependent} regret guarantees for Algorithm~\ref{alg:dUCB} for both the estimators proposed. For the clipped estimator~\eqref{eq:est1}, the regret scales as $\mathcal{O}\left(\mathcal{M}\left( \pmb{\mu},\{M_{ij}\} \right) \log T \right)$, where $\mathcal{M}\left(\pmb{\mu},\{M_{ij}\}\right)$ is an instance dependent term that depends on the mean reward gaps between the experts and log-divergences. We will show that the regret typically scales as $\mathcal{O}(M^2\log N \log^3 T/\Delta)$ under some assumptions, where $\Delta = \min_{k \neq k^*} \Delta_k$ and $M$ is the maximum log-divergence between two experts. 

Similarly, we will show that the regret of Algorithm~\ref{alg:dUCB} using the median of means estimator~\eqref{eq:est2}, scales as $\mathcal{O}\left(\mathcal{S}\left(\pmb{\mu},\{\sigma_{ij}\}\right) \log T \right)$. Here, $\mathcal{S}\left(\pmb{\mu},\{\sigma_{ij}\}\right)$ is an instance dependent term that depends on the mean reward gaps between the experts and chi-square-divergences. We will show that this term typically scales as $\mathcal{O}(\sigma^2\log N/\Delta)$ under some assumptions, where $\sigma$ is the maximum chi-square divergence between two experts.

In contrast, if the experts were used as separate arms, a naive application of UCB-1~\cite{auer2002using} bounds would yield a regret scaling of $\mathcal{O} \left(\frac{N}{\Delta} \log T \right)$. This can be prohibitively large when the number of experts are large.  

For ease of exposition of our results, let us re-index the experts using indices $\{(1),(2),...,(N) \}$ such that $0 = \Delta_{(1)} \leq \Delta_{(2)} \leq ... \leq \Delta_{(N)}$. The regret guarantees for our clipped estimator are provided under the following assumption. 

\begin{assumption}
	\label{assump1}
	We assume the log-divergence terms~\eqref{def:mij} are bounded for all $i,j \in [N]$. Let $M = \max_{i,j} M_{ij}$. 
\end{assumption}

Now we are at a position to present one of our main theorems that provides regret guarantees for Algorithm~\ref{alg:dUCB} using the estimator~\eqref{eq:est1}. 

\begin{theorem}
	\label{thm:r1}
	Suppose Assumption~\ref{assump1} holds. Then the regret of Algorithm~\ref{alg:dUCB} at time $T$ using estimator~\eqref{eq:est1},  is bounded as follows:
	\begin{align*}
	&R(T) \leq \frac{C_1M^2 \log^2 (6/\Delta _{(N)}) \log T}{\Delta_{(N)}} + \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right) \\
	&+  \sum_{k = 2}^{N-1} \frac{C_1M^2 \log^2 (6/\Delta _{(k)}) \log T}{\Delta_{(k)}} \left(1 - \frac{\gamma(\Delta_{(k)})}{\gamma(\Delta_{(k+1)})} \right) \\
	& \leq \frac{C_1M^2 \log^2 (6/\Delta _{(2)}) \log T}{\Delta_{(2)}} \left(1  \right. \\
	&\left. +\sum_{k = 2}^{N-1} \left(1 - \frac{\gamma(\Delta_{(k)})}{\gamma(\Delta_{(k+1)})} \right) \right) + \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right).
	\end{align*}
	Here, $C_1$ is an universal constant and $\gamma(x) = \frac{x^2}{\log ^2 (6/x)}$.
\end{theorem}

We defer the proof of Theorem~\ref{thm:r1} to Appendix~\ref{sec:clipped}. We now present Theorem~\ref{thm:r2} that provides regret guarantees for Algorithm~\ref{alg:dUCB} using the estimator~\eqref{eq:est2}. The theorem holds under the following assumption. 

\begin{assumption}
	\label{assump2}
	We assume the chi-square-divergence terms~\eqref{def:sij} are bounded for all $i,j \in [N]$. Let $\sigma = \max_{i,j} \sigma_{ij}$. 
\end{assumption}

\begin{theorem}
	\label{thm:r2}
	Suppose Assumption~\ref{assump2} holds. Then the regret of Algorithm~\ref{alg:dUCB} at time $T$ using estimator~\eqref{eq:est2},  is bounded as follows:
	\begin{align*}
	&R(T) \leq \frac{C_2\sigma^2 \log T}{\Delta_{(N)}} \\
	&+  \sum_{k = 2}^{N-1} \frac{C_2\sigma^2 \log T}{\Delta_{(k)}} \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) + \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right) \\
	& \leq \frac{C_2\sigma^2 \log T}{\Delta_{(2)}} \left(1 + \sum_{k = 2}^{N-1} \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) \right) \\
	&+ \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right).
	\end{align*}
	Here, $C_2$ is an universal constant. 
\end{theorem}

The proof of Theorem~\ref{thm:r2} has been deferred to Appendix~\ref{sec:mom}. Now, we will delve deeper into the instance dependent terms in Theorems~\ref{thm:r1} and~\ref{thm:r2}. First, we have the following corollary (that follows trivially from Theorem~\ref{thm:r1} and \ref{thm:r2}), which states that we can achieve regret bounds without any dependence on $N$, but $\mathcal{O}(1/\Delta_{(2)}^2)$ dependence on the smallest gap.  
\begin{corollary}
	\label{cor:delta}
	We have the following regret bound for Algorithm~\ref{alg:dUCB}: 
	
	($i$) Under estimator~\eqref{eq:est1}, 
	
	$R(T) = \mathcal{O} \left(\frac{M^2 \log^2 (1/\Delta_{(2)}) \log T}{\Delta_{(2)}^2} \right)$.
	
	($ii$) Under estimator~\eqref{eq:est2}, $R(T) = \mathcal{O} \left(\frac{\sigma^2 \log T}{\Delta_{(2)}^2} \right)$. 
\end{corollary}

Now, we will show that when the gaps $\Delta$'s are uniformly distributed then the instance dependent terms approximately scale as $\mathcal{O} \left(\log N / \Delta_{(2)} \right)$, in expectation. 

\begin{lemma}
	\label{lem:mu}
	Consider a generative model where $\Delta_{(3)}\leq...\leq\Delta_{(N)}$ are the order statistics of $N-2$ random variables drawn i.i.d uniform over the interval $[\Delta_{(2)},1]$. Let $p_{\Delta}$ denote the measure over these $\Delta$'s. Then we have the following:
	
	($i$) For Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est1}, 
	
	$\EE_{p_{\Delta}} \left[ R(T)\right] = \mathcal{O} \left(\frac{M^2 \log N \log^3 T }{\Delta_{(2)}} \right)$, if $\Delta_{(2)} > 1/T$. 
	
	($ii$) For Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est2}, 
	
	$\EE_{p_{\Delta}} \left[ R(T)\right] = \mathcal{O} \left(\frac{\sigma^2 \log N \log T }{\Delta_{(2)}} \right)$.
\end{lemma}

\begin{remark}
Note that our guarantees do not have any term containing $K$ - the number of arms. This dependence is implicitly captured in the divergence terms among the experts. In fact when the number of arms $K$ is very large, we expect our divergence based algorithms to perform comparatively better than other algorithms, whose guarantees explicitly depend on $K$. This phenomenon is observed in practice in our empirical validation on real world data-sets in Section~\ref{sec:sims}. 
\end{remark}





==> resultsv2.tex <==
\section{Theoretical Results}
\label{sec:results}
In this section we provide \textit{instance dependent} regret guarantees for Algorithm~\ref{alg:dUCB} for both the estimators proposed. For the clipped estimator~\eqref{eq:est1}, the regret scales as $\mathcal{O}\left(\mathcal{M}\left( \pmb{\mu},\{M_{ij}\} \right) \log T \right)$, where $\mathcal{M}\left(\pmb{\mu},\{M_{ij}\}\right)$ is an instance dependent term that depends on the mean reward gaps between the experts and log-divergences. We will show that the regret typically scales as $\mathcal{O}(M^2\log N \log^2(1/\Delta) \log T/\Delta)$ in expectation, under some assumptions, where $\Delta = \min_{k \neq k^*} \Delta_k$ and $M$ is the maximum log-divergence between two experts. 

Similarly, we will show that the regret of Algorithm~\ref{alg:dUCB} using the median of means estimator~\eqref{eq:est2}, scales as $\mathcal{O}\left(\mathcal{S}\left(\pmb{\mu},\{\sigma_{ij}\}\right) \log T \right)$. Here, $\mathcal{S}\left(\pmb{\mu},\{\sigma_{ij}\}\right)$ is an instance dependent term that depends on the mean reward gaps between the experts and chi-square-divergences. We will show that this term typically scales as $\mathcal{O}(\sigma^2\log N/\Delta)$ under some assumptions, where $\sigma$ is the maximum chi-square divergence between two experts.

In contrast, if the experts were used as separate arms, a naive application of UCB-1~\cite{auer2002using} bounds would yield a regret scaling of $\mathcal{O} \left(\frac{N}{\Delta} \log T \right)$. This can be prohibitively large when the number of experts are large.  

For ease of exposition of our results, let us re-index the experts using indices $\{(1),(2),...,(N) \}$ such that $0 = \Delta_{(1)} \leq \Delta_{(2)} \leq ... \leq \Delta_{(N)}$. The regret guarantees for our clipped estimator are provided under the following assumption. 

\begin{assumption}
	\label{assump1}
	We assume the log-divergence terms~\eqref{def:mij} are bounded for all $i,j \in [N]$. Let $M = \max_{i,j} M_{ij}$. 
\end{assumption}

Now we are at a position to present one of our main theorems that provides regret guarantees for Algorithm~\ref{alg:dUCB} using the estimator~\eqref{eq:est1}. 

\begin{theorem}
	\label{thm:r1}
	Suppose Assumption~\ref{assump1} holds. Then the regret of Algorithm~\ref{alg:dUCB} at time $T$ using estimator~\eqref{eq:est1},  is bounded as follows:
	\begin{align*}
	&R(T) \leq \frac{C_1M^2 \log^2 (6/\Delta _{(N)}) \log T}{\Delta_{(N)}} + \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right) \\
	&+  \sum_{k = 2}^{N-1} \frac{C_1M^2 \log^2 (6/\Delta _{(k)}) \log T}{\Delta_{(k)}} \left(1 - \frac{\gamma(\Delta_{(k)})}{\gamma(\Delta_{(k+1)})} \right) 
	\end{align*}
	Here, $C_1$ is an universal constant and $\gamma(x) = \frac{x^2}{\log ^2 (6/x)}$.
\end{theorem}

We defer the proof of Theorem~\ref{thm:r1} to Appendix~\ref{sec:clipped}. We now present Theorem~\ref{thm:r2} that provides regret guarantees for Algorithm~\ref{alg:dUCB} using the estimator~\eqref{eq:est2}. The theorem holds under the following assumption. 

\begin{assumption}
	\label{assump2}
	We assume the chi-square-divergence terms~\eqref{def:sij} are bounded for all $i,j \in [N]$. Let $\sigma = \max_{i,j} \sigma_{ij}$. 
\end{assumption}

\begin{theorem}
	\label{thm:r2}
	Suppose Assumption~\ref{assump2} holds. Then the regret of Algorithm~\ref{alg:dUCB} at time $T$ using estimator~\eqref{eq:est2},  is bounded as follows:
	\begin{align*}
	&R(T) \leq \frac{C_2\sigma^2 \log T}{\Delta_{(N)}} \\
	&+  \sum_{k = 2}^{N-1} \frac{C_2\sigma^2 \log T}{\Delta_{(k)}} \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) + \frac{\pi^2}{3} \left(\sum_{i = 2}^{N} \Delta_{(i)} \right) 
	\end{align*}
	Here, $C_2$ is an universal constant. 
\end{theorem}

The proof of Theorem~\ref{thm:r2} has been deferred to Appendix~\ref{sec:mom}. Now, we will delve deeper into the instance dependent terms in Theorems~\ref{thm:r1} and~\ref{thm:r2}. The proofs of Theorem~\ref{thm:r1} and \ref{thm:r2} imply the following corollary.

\begin{corollary}
	\label{cor:simple}
	Let $\lambda(\pmb{\mu}) \triangleq \sum_{k = 2}^{N-1}  \left(1 - \frac{\Delta_{(k)}^2}{\Delta_{(k+1)}^2} \right) $. We have the following regret bounds: 
	
	$(i)$ For Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est1}, 
	
	$R(T) \leq  \mathcal{O} \left(\frac{\lambda(\pmb{\mu}) M^2 \log^2 (6/\Delta _{(2)}) \log T}{\Delta_{(2)}} \right)$. 
	
	$(ii)$ Similarly for Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est2}, $R(T) \leq  \mathcal{O} \left(\frac{\lambda(\pmb{\mu}) \sigma^2  \log T}{\Delta_{(2)}} \right)$
\end{corollary} 

Corollary~\ref{cor:simple} leads us to our next result. In Corollary~\ref{lem:mu} we show that when the $\Delta$ gaps are uniformly distribution, then the term $\lambda(\pmb{\mu})$ scales as $O(\log N)$, in expectation.

 
\begin{corollary}
	\label{lem:mu}
	Consider a generative model where $\Delta_{(3)}\leq...\leq\Delta_{(N)}$ are the order statistics of $N-2$ random variables drawn i.i.d uniform over the interval $[\Delta_{(2)},1]$. Let $p_{\Delta}$ denote the measure over these $\Delta$'s. Then we have the following:
	
	($i$) For Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est1}, 
	
	$\EE_{p_{\Delta}} \left[ R(T)\right] = \mathcal{O} \left(\frac{M^2 \log N \log^2(1/\Delta_{(2)}) \log T }{\Delta_{(2)}} \right)$.
	
	($ii$) For Algorithm~\ref{alg:dUCB} with estimator~\eqref{eq:est2}, 
	
	$\EE_{p_{\Delta}} \left[ R(T)\right] = \mathcal{O} \left(\frac{\sigma^2 \log N \log T }{\Delta_{(2)}} \right)$.
\end{corollary}

In Corollary~\ref{cor:delta}, we display an alternative bound for the regret of Algorithm~\ref{alg:dUCB}. We show that it is possible to avoid the dependence in $N$ altogether however at the cost of scaling $O(1/\Delta_{(2)}^2)$ in the minimum gap.  
\begin{corollary}
	\label{cor:delta}
	We have the following regret bound for Algorithm~\ref{alg:dUCB}: 
	
	($i$) Under estimator~\eqref{eq:est1}, 
	
	$R(T) = \mathcal{O} \left(\frac{M^2 \log^2 (1/\Delta_{(2)}) \log T}{\Delta_{(2)}^2} \right)$.
	
	($ii$) Under estimator~\eqref{eq:est2}, $R(T) = \mathcal{O} \left(\frac{\sigma^2 \log T}{\Delta_{(2)}^2} \right)$. 
\end{corollary}



\begin{remark}
Note that our guarantees do not have any term containing $K$ - the number of arms. This dependence is implicitly captured in the divergence terms among the experts. In fact when the number of arms $K$ is very large, we expect our divergence based algorithms to perform comparatively better than other algorithms, whose guarantees explicitly depend on $K$. This phenomenon is observed in practice in our empirical validation on real world data-sets in Section~\ref{sec:sims}. 
\end{remark}




